Generalized cluster structures related to Poisson duals of $\mathrm{SL}_n$

We study Poisson varieties $(\mathrm{SL}_n,\pi_{\bar{\mathbf{\Gamma}}}^{\dagger})$ parameterized by Belavin--Drinfeld quadruples $\bar{\mathbf{\Gamma}}:=(\mathbf{\Gamma},r_0)$ of type $A_{n-1}$ along with generalized cluster structures $\mathcal{GC}^{\dagger}(\mathbf{\Gamma})$ in $\mathbb{C}[\mathrm{SL}_n]$ compatible with $\pi_{\bar{\mathbf{\Gamma}}}^{\dagger}$. The Poisson structure $\pi_{\bar{\mathbf{\Gamma}}}^{\dagger}$ is a pushforward of the Poisson structure $\pi_{\bar{\mathbf{\Gamma}}}^*$ of the Poisson dual $\mathrm{SL}_n^*$ of $(\mathrm{SL}_n,\pi_{\bar{\mathbf{\Gamma}}})$. We prove that the generalized upper cluster algebra of $\mathcal{GC}^{\dagger}(\mathbf{\Gamma})$ is naturally isomorphic to $\mathbb{C}[\mathrm{SL}_n]$. Moreover, for any connected reductive complex group $G$ and a BD quadruple $(\mathbf{\Gamma},r_0)$, we produce a Poisson birational map $\mathcal{Q}:(G,\pi_{(\mathbf{\Gamma}_{\text{std}},r_0)}^{\dagger})\dashrightarrow(G,\pi_{(\mathbf{\Gamma},r_0)}^{\dagger})$, and when $G \in \{\mathrm{SL}_n,\mathrm{GL}_n\}$, we show that $\mathcal{Q}$ is a birational quasi-isomorphism between $\mathcal{GC}^\dagger(\mathbf{\Gamma}_{\text{std}})$ and $\mathcal{GC}^\dagger(\mathbf{\Gamma})$. Lastly, for any pair of BD triples $\tilde{\mathbf{\Gamma}} \prec \mathbf{\Gamma}$ of type $A_{n-1}$ comparable in the natural order, we use the map $\mathcal{Q}$ to construct a birational quasi-isomorphism between $\mathcal{GC}^{\dagger}(\tilde{\mathbf{\Gamma}})$ and $\mathcal{GC}^{\dagger}(\mathbf{\Gamma})$.

==> c_comp_final.tex <==
In this subsection, we use the Poisson properties established for the birational quasi-isomorphism $\mathcal{Q}$ in order to conclude that $\gc_h^{\dagger}(\bg)$ is compatible with $\pi^{\dagger}_{\bg}$ for any BD triple $\bg$ of type~$A_{n-1}$.

\begin{lemma}\label{l:compmarked}
    Let $\bg:=(\Gamma_1,\Gamma_2,\gamma)$ be a BD triple such that $\Gamma_1 = \{p\}$, $\Gamma_2 = \{q\}$ for some simple roots $p$ and $q$. Then for any cluster or frozen variable $\psi$ from the initial extended cluster of $\gc^{\dagger}(\bg)$,
    \[
    \{\log y(h_{q+1,q+1}), \log \psi\} = \begin{cases}
        1 \ &\text{if} \ \psi = h_{q+1,q+1},\\
        0 \ &\text{otherwise.}
    \end{cases}
    \]
\end{lemma}
\begin{proof}
Set $\psi_{\square}:=h_{q+1,q+1}$. Let us recall that in the case we consider $\gc_h(\bg)$ and $\gc_h(\bg_{\std})$ at once, the $h$-variables in the latter are embellished with a tilde (see the preamble to Section~\ref{s:birat}). Let us apply the birational quasi-isomorphism $\mathcal{Q}$ and prove an equivalent statement for the trivial BD triple. We see that\footnote{Note: since $\tilde{\psi}_{\square}$ is frozen in $\gc^{\dagger}_{h}(\bg_{\std})$, $\mathcal{Q}^*(y(\psi_{\square}))$ is not a $y$-variable.}
\begin{equation}
    \mathcal{Q}^* (y(\psi_{\square})) = \frac{\tilde{h}_{qq}}{\tilde{h}_{q,q+1}} \frac{\tilde{h}_{pn}}{\tilde{h}_{p+1,n}}\frac{\tilde{h}_{q+1,q+2}}{\tilde{h}_{q+1,q+1}}.
\end{equation}
Let us first consider the case when $\psi$ is an $h$-variable. If $h_1$ and $h_2$ are two functions on $\GL_n$ such that $h_i(UN_-) = h_i(U)$, where $N_-$ is a unipotent lower triangular matrix, $i \in \{1,2\}$, then the Poisson bracket $\{\cdot,\cdot\}_{\std}^{\dagger}$ between them is given by
\begin{equation}
\{h_1,h_2\}_{\std}^{\dagger} = \langle \pi_{>} \nabla_U^R h_1,\nabla_U^R h_2\rangle + \langle R_0[\nabla_U h_1,U],[\nabla_U h_2,U]\rangle - \langle \pi_0[\nabla_U h_1,U],\nabla_U h_2 U\rangle.
\end{equation}
It follows from Lemma~\ref{l:grrhijks} that 
%\begin{equation}
%\langle \pi_{>}\left( \nabla_U^R \log \frac{\tilde{h}_{pn}}{\tilde{h}_{p+1,n}}\right),\nabla_U^R \log \tilde{h}_{ks} \rangle = \begin{cases}
%-1 \ &\text{if} \ n-s = p-k,\\
%0 \ &\text{otherwise;}
%\end{cases}
%\end{equation}
%\begin{equation}
%\langle \pi_{>}\left(\nabla_U^R \log \frac{\tilde{h}_{qq}}{\tilde{h}_{q,q+1}}\frac{\tilde{h}_{q+1,q+2}}{\tilde{h}_{q+1,q+1}}  \right), \nabla_U^R \log \tilde{h}_{ks}\rangle = \begin{cases}
%-1 \ &\text{if} \ k \leq q \ \text{and} \ s = q+1,\\
%0 \ &\text{otherwise.}
%\end{cases}
%\end{equation}
\begin{equation}
\langle \pi_{>}\left( \nabla_U^R \log \frac{\tilde{h}_{pn}}{\tilde{h}_{p+1,n}}\right),\nabla_U^R \log \tilde{h}_{ks} \rangle = -\chi_{n-s=p-k}
\end{equation}
\begin{equation}
\langle \pi_{>}\left(\nabla_U^R \log \frac{\tilde{h}_{qq}}{\tilde{h}_{q,q+1}}\frac{\tilde{h}_{q+1,q+2}}{\tilde{h}_{q+1,q+1}}  \right), \nabla_U^R \log \tilde{h}_{ks}\rangle = -\chi_{k \leq q}\cdot \chi_{s = q+1}
\end{equation}
where $\chi_{(\cdot)} \in \{0,1\}$ is an indicator that returns true or false depending on whether the corresponding condition is satisfied. It follows from Lemma~\ref{l:hijlrd} that
\begin{equation}\label{eq:gradqyps}
\pi_0\left( \nabla_U^L \log \mathcal{Q}^* y(\psi_{\square}) \right) = e_{qq}-e_{q+1,q+1}, \ \ \pi_0\left( \nabla_U^R \mathcal{Q}^* y(\psi_{\square}) \right) = e_{pp}-e_{p+1,p+1},
\end{equation}
hence
\begin{equation}\label{eq:r0qypsi}\begin{split}
R_0[\nabla_U \log \mathcal{Q}^*& y(\psi_{\square}),U] = R_0(e_{qq}-e_{q+1,q+1} - (e_{pp}-e_{p+1,p+1})) = \\=&-R_0(1-\gamma)(e_{pp}-e_{p+1,p+1}) = -e_{pp}+e_{p+1,p+1}.
\end{split}
\end{equation}
Let us set $\Delta(i,j) := \sum_{t = i}^{j} e_{ii}$. We see that
\begin{equation}\label{eq:lastbraq}
\begin{split}
\{\log \mathcal{Q}^*y(\psi_{\square}), \log \hat{h}_{ks}\}_{\std}^{\dagger} = &-\chi_{n-s=p-k} - \chi_{k \leq q}\cdot \chi_{s = q+1} +\\+& \langle e_{pp}-e_{p+1,p+1},\Delta(k,n-s+k) \rangle - \langle e_{qq}-e_{q+1,q+1}, \Delta(s,n) \rangle = \\ = &-\chi_{k = p+1}+ (1-\chi_{k\leq q})\chi_{s=q+1} = -\chi_{k = p+1}+\chi_{k=q+1}\chi_{s=q+1}.
\end{split}
\end{equation}
Now let us recall that $\mathcal{Q}^*({h_{ks}}) = \tilde{h}_{ks}$ if $k \neq p+1$ and $\mathcal{Q}^*(h_{p+1,s}) = \tilde{h}_{p+1,s}\tilde{h}_{q+1,q+1}$. With the latter and Formula~\eqref{eq:lastbraq}, the result follows in the case $\psi$ is an $h$-function. As for the other case, if $h$ is a function such that $h(UN_-) = h(U)$, then for any $\varphi$-function $\varphi_{kl}$,
\begin{equation}
\{\log h,\log \varphi_{kl}\}_{\std}^{\dagger} = \langle R_0[\nabla_U \log h,U],[\nabla_U\log \varphi_{kl},U]\rangle - \langle \pi_0 \nabla_U^R \log h,[\nabla_U\log \varphi_{kl},U]\rangle.
\end{equation}
Setting $h:=\log \mathcal{Q}^*y(\psi_{\square})$ and applying $\pi_0[\nabla_U\log \varphi_{kl},U] = \const$ together with \eqref{eq:gradqyps} and \eqref{eq:r0qypsi}, we obtain that 
\[
\{\log \mathcal{Q}^*y(\psi_{\square}),\log \varphi_{kl}\}_{\std}^{\dagger} = 0. 
\]
Thus the result follows.
\end{proof}

%\begin{lemma}
%Let $\bg$ be any BD triple of type $A_{n-1}$, and let $r_0$ and $r_0^\prime$ be two different $r_0$ elements that correspond to $\bg$. We set $\pi_{\bg,r_0}^{\dagger}$ and $\pi_{\bg,r_0^\prime}^{\dagger}$ to be the corresponding bivectors. If $\gc_h(\bg)$ is compatible with $\pi_{\bg,r_0}^{\dagger}$, then it is compatible with $\pi_{\bg,r_0^{\prime}}^{\dagger}$ as well. %If an extended cluster $\Psi$ in $\gc_h^{\dagger}(\bg)$ is log-canonical relative $\pi_{\bg,r_0}^{\dagger}$, then it is log-canonical with respect to $\pi_{\bg,r_0^{\prime}}^{\dagger}$ as well. In particular, if $\gc_h^{\dagger}(\bg)$ is compati 
%\end{lemma}
%\begin{proof}
%Let $\Psi = (\psi_1,\psi_2,\ldots,\psi_m)$ be an extended cluster in $\gc_h^{\dagger}(\bg)$. 
%\end{proof}

\begin{proposition}\label{p:compatibl}
Let $\bg$ be any BD triple of type $A_{n-1}$. For any choice of $r_0$ relative the triple $\bg$, the generalized cluster structure $\gc_h^{\dagger}(\bg)$ is compatible with $\pi_{\bg}^{\dagger}$.
\end{proposition}
\begin{proof}
Let us fix $n$ and run an induction on the size $|\Gamma_1|$. For $|\Gamma_1| = 0$, this is a consequence of the work~\cite{double}. Let $\bg$ be any BD triple of type $A_{n-1}$ and $\tilde{\bg}$ be the BD triple obtained from $\bg$ via removal of $p \in \Gamma_1$ and $q \in \Gamma_2$. Let $\mathcal{G}:(G,\pi_{\tilde{\bg}}^{\dagger}) \dashrightarrow (G,\pi_{\bg}^{\dagger})$ be the birational quasi-isomorphism constructed in Section~\ref{s:bsimpl}, where $G \in \{\SL_n,\GL_n\}$. Let $\tilde{\Psi}_0$ and $\Psi_0$ be the initial extended clusters of $\gc_h^{\dagger}(\tilde{\bg},G)$ and $\gc_h^{\dagger}(\bg,G)$, and let $\psi_{\square} \in \Psi_0$ be the marked variable. Since $\tilde{\bg} \preceq \bg$, any $r_0$ element for $\pi_{\bg}^{\dagger}$ is also an $r_0$ element for $\pi_{\tilde{\bg}}^{\dagger}$; hence, we choose the same $r_0$ to make $\mathcal{G}$ a Poisson isomorphism (see Corollary~\ref{c:gpoiss}). Now, since $\tilde{\Psi}_0$ is assumed to be log-canonical and $\mathcal{G}$ is a Poisson isomorphism, $\Psi$ is log-canonical as well. Let $\psi_1 \in \Psi_0\setminus \{\psi_{\square}\}$ be a cluster variable and $\psi_2 \in \Psi_0$ be any cluster or frozen variable. Since
\[
\{\log y(\tilde{\psi}_1),\log \tilde{\psi}_2\} = \chi_{\tilde{\psi}_1 = \tilde{\psi}_2},
\]
an application of $(\mathcal{G}^*)^{-1}$ yields
\begin{equation}\label{eq:ypsir}
\{\log y(\psi_1),\log \psi_2\} = \chi_{\psi_1 = \psi_2}.
\end{equation}
Now, if $|\Gamma_1| = 1$, it follows from Lemma~\ref{l:compmarked} (which treats the case of $\psi_1 = \psi_{\square}$) and Proposition~\ref{p:compb} that $\gc_h^{\dagger}(\bg,G)$ is compatible with $\pi_{\bg}^{\dagger}$. For $|\Gamma_1| = 1$, to verify~\eqref{eq:ypsir} for the marked variables, one can use another birational quasi-isomorphism $\mathcal{G}$ whose marked variables are disjoint from the former one (i.e., remove a different pair of roots from $\bg$). Thus the statement of the proposition holds.
\end{proof}

==> completeness.tex <==
In this section, we prove that the generalized upper cluster structure of $\gc_h^{\dagger}(\bg,\GL_n)$ is naturally isomorphic to the ring of regular functions $\mathbb{C}[\GL_n]$. Along the way, we will prove that all the variables in the initial extended cluster are irreducible (as elements of $\mathbb{C}[\GL_n]$) and (for the initial cluster variables) coprime with their mutations.

%%Let $\bg_{\std}$ be the standard Belavin-Drinfeld triple, and let us embellish the $h$-variables in $\gc_h^{\dagger}(\bg_{\std})$ with a tilde (i.e., write $\tilde{h}_{ij}(U)$), to distinguish them from the $h$-variables in $\gc_h^{\dagger}(\bg)$. Consider the birational quasi-isomorphism $\mathcal{Q}:(\GL_n)_{\std} \dashrightarrow (\GL_n)_{\bg}$ constructed via Formula~\eqref{eq:defqq}. In the terminology of Definition~\ref{d:marked}, $\gc_h^{\dagger}(\bg)$ and $\gc_h^{\dagger}(\bg_{\std})$ are related, and the marker is given by assigning each variable $\varphi_{ij}(U)$ and $c_k(U)$ to itself, and each $h_{ij}(U)$ to $\tilde{h}_{ij}(U)$ (in the initial extended clusters). Then $\psi_{\square}(U):=h_{q+1,q+1}(U)$ is the marked variable. The birational isomorphism $\mathcal{F}^c = \mathcal{Q}^{-1}$ assumes the form

\subsection{The case of $|\Gamma_1|=|\Gamma_2| = 1$ (shifted cluster).}
Let $\bg = (\Gamma_1,\Gamma_2,\gamma)$ be a Belavin-Drinfeld of type $A_{n-1}$ such that $\Gamma_1:=\{p\}$ and $\Gamma_2:=\{q\}$ for some simple roots $p$ and $q$. Let $\tilde{\bg}$ be the standard Belavin-Drinfeld triple. We embellish the $h$-variables in $\gc_h^{\dagger}(\bg_{\std})$ with a tilde, to distinguish them from the $h$-variables in $\gc_h^{\dagger}(\bg)$. Recall that we choose the marker (see Definition~\ref{d:marker}) between $\gc_{h}^{\dagger}(\tilde{\bg})$ and $\gc_h^{\dagger}(\bg)$ in such a way that each $\varphi$- and $c$- variable is related to itself, and each $h_{ij}$ is related to $\tilde{h}_{ij}$. We also consider the birational quasi-isomorphism $\mathcal{Q}:(\GL_n,\pi_{\std}^{\dagger}) \dashrightarrow (\GL_n,\pi_{\bg}^{\dagger})$ constructed in Section~\ref{s:birat}. In this case, the marked variable is given by $\psi_{\square}:=h_{q+1,q+1}$. The map $\mathcal{F}^c = \mathcal{Q}^{-1}$ assumes the form
\begin{equation}\label{eq:fcbase}
\mathcal{F}^c(U) = \tilde{\gamma}^*(U_-) U \tilde{\gamma}^*(U_-)^{-1}, \ \ \tilde{\gamma}^*(U_-) = I + \alpha(U)e_{p+1,p}, \ \ \alpha(U) = \frac{1}{\psi_{\square}(U)}\det U^{\{q\}\cup[q+2,n]}_{[q+1,n]}.
\end{equation}

\paragraph{Shifting the initial cluster.} We will prove $\bar{\mathcal{A}}_{\mathbb{C}}(\gc_h^{\dagger}(\bg)) = \mathbb{C}[\GL_n]$ starting not in the initial extended cluster, but in a more convenient one. Let us set $\Psi$ to be the extended cluster in $\gc_h^{\dagger}(\bg)$ obtained via applying the following mutation sequence\footnote{If $p = n-1$, the mutation sequence is empty, so  we set $\Psi$ to be the initial extended cluster.} to the initial extended cluster:
\[
{h}_{p+1,n} \rightarrow {h}_{p+1,n-1} \rightarrow \cdots \rightarrow {h}_{p+1,p+2}.
\]
We set $\tilde{\Psi}$ to be the extended cluster in $\gc_h^{\dagger}(\bg_{\std})$ related to $\Psi$ (see Definition~\ref{d:marked}) and $\Psi^{\prime}$ to be the extended cluster in $\gc_h^{\dagger}(\bg)$ obtained by mutating $\Psi$ in the direction of $\psi_{\square}$. 

\begin{lemma}\label{l:relpsi}
    The extended cluster $\Psi$ contains the variables
    \begin{equation}\label{eq:hpps}
    {h}^{\prime}_{p+1,n-s}(U) = -(-1)^{s(n-(p+1))} \det U_{\{p\}\cup[p+2,s+p+2]}^{[n-s-1,n]}, \ \ s \in [0,n-p-2].
    \end{equation}
    In particular, for any $\psi \in \Psi\setminus\{h_{p+1,p+1}\}$ and the related variable $\tilde{\psi} \in \tilde{\Psi}\setminus\{\tilde{h}_{p+1,p+1}\}$, \mbox{$\tilde{\psi}(U) = \psi(U)$}.
\end{lemma}
\begin{proof}
It is well-known (see, for instance, Lemma 5.3 in~\cite{multdouble}, with adjustments to signs) that $\tilde{\Psi}$ contains the variables
    \begin{equation}\label{eq:thpps}
    {h}^{\prime}_{p+1,n-s}(U) = -(-1)^{s(n-(p+1))} \det U_{\{p\}\cup[p+2,s+p+2]}^{[n-s-1,n]}, \ \ s \in [0,n-p-2].
    \end{equation}
Applying $(\mathcal{F}^c)^*$ to~\eqref{eq:thpps}, we see that
\[\begin{split}
(\mathcal{F}^c)^*[\tilde{h}^{\prime}_{p+1,n-s}(U)] = -&(-1)^{s(n-(p+1))} \det [\tilde{\gamma}^*(U_-)U]_{\{p\}\cup[p+2,s+p+2]}^{[n-s-1,n]} =\\= -&(-1)^{s(n-(p+1))} \det U_{\{p\}\cup[p+2,s+p+2]}^{[n-s-1,n]},
\end{split}
\]
where $\tilde{\gamma}^*(U_-) = I + \alpha(U)e_{p+1,p}$ for some $\alpha$, and hence $\tilde{\gamma}^*(U_-)$ can be removed from the determinant. Since $\mathcal{Q}$ is a quasi-isomorphism, we conclude that the related extended cluster $\Psi$ contains the variables~\eqref{eq:hpps}. In particular, $\Psi$ and $\tilde{\Psi}$ differ only in the variable $h_{p+1,p+1}$.
\end{proof}

% For the next lemma, let us adopt the following conventions:
% \begin{equation}\label{eq:hconv}
% h_{1j}(U) := \varphi_{j-1,n-j+1}(U) = (-1)^{\varepsilon_{1j}}\det U^{[j,n]}_{[1,n-j+1]}, \ \ j \in [2,n];
% \end{equation}
% \begin{equation}\label{eq:hconv2}
% h_{i,n+1}(U) = 1, \ \ i \in [1,n];
% \end{equation}
% where $\varepsilon_{1j}$ is given by~\eqref{eq:h_sign}. Let us also mention that
For the next lemma, let us mention that the frozen variable $h_{p+1,p+1}$ in $\gc_h^{\dagger}(\bg)$ is given by 
\begin{equation}\label{eq:hp1p1}
h_{p+1,p+1}(U) = \det U^{[p+1,n]}_{[p+1,n]} \det U^{[q+1,n]}_{[q+1,n]} + \det U^{[p+1,n]}_{\{p\}\cup [p+2,n]} \det U^{\{q\}\cup[q+2,n]}_{[q+1,n]}.
\end{equation} 
This can be obtained either via the explicit Formula~\eqref{eq:halphao} or via Formula~\eqref{eq:h_fun_enh} by expanding
\[
h_{p+1,p+1}(U) = \det [\tilde{\gamma}^*(U_-)U]_{[p+1,n]}^{[p+1,n]} \det U^{[q+1,n]}_{[q+1,n]}.
\]

\begin{lemma}
The mutation of $\Psi$ at the marked variable $\psi_{\square}$ produces the variable
\begin{equation}\label{eq:psisqm}
\psi_{\square}^{\prime}(U) = (-1)^{\varepsilon_{\square}} \left[\det U^{[p+1,n]}_{[p+1,n]} \det U_{I_{\square}}^{[q+1,n]} + \det U^{[p+1,n]}_{\{p\}\cup [p+2,n]} \det U^{\{q\}\cup[q+2,n]}_{I_{\square}}\right]
\end{equation}
where 
\begin{equation}\label{eq:intsq}
\varepsilon_{\square} := \begin{cases} n-q \ &\text{if}\ q-p\neq 1,\\ n-q+1 \ &\text{if} \ q-p = 1; \end{cases} \ \ \  I_{\square} := \begin{cases}
[q,n-1] \ &\text{if} \ q-p \neq 1,\\
\{q-1\}\cup[q+1,n-1] \ &\text{if} \ q-p=1.
\end{cases}
\end{equation}
%Moreover, both $\psi_{\square}(U)$ and $\psi_{\square}^{\prime}(U)$ are irreducible as elements of $\mathbb{C}[\GL_n]$.
\end{lemma}
\begin{proof}
\emph{Case $q-p = 1$, $q \leq n-2$.} The mutation relation for $\psi_{\square}$ reads
\begin{equation}
\psi_{\square}\psi_{\square}^{\prime} = (h_{p+1,p+2}^\prime)^2 h_{q+1,q+2} + h_{p+1,p+3}^\prime h_{p+1,p+1}.
\end{equation}
Expanding the right-hand side, we see that
\begin{equation}\label{eq:complcso}
\begin{split}
(-1)^{n-p} &\psi_{\square}(U)\psi_{\square}^{\prime}(U) = \left[\det U^{[p+1,n]}_{\{p\}\cup[p+2,n]}\right]^{2} \det U^{[p+3,n]}_{[p+2,n]} +\\ +  &\det U^{[p+2,n]}_{\{p\}\cup [p+2,n-1]} \left[ \det U^{[p+1,n]}_{[p+1,n]} \det U^{[q+1,n]}_{[q+1,n]} + \det U^{\{q\}\cup [q+2,n]}_{[q+1,n]} \det U^{[p+1,n]}_{\{p\}\cup [p+2,n]} \right].
\end{split}
\end{equation}
Applying the Desnanot-Jacobi identity (see Proposition~\ref{p:dj22}) to the matrix $A:= U^{[p+1,n]}_{\{p\}\cup[p+2,n]}$, we see that
\begin{equation}\label{eq:compldj}\begin{split}
\det U^{[p+1,n]}_{\{p\}\cup[p+2,n]} \det U^{[p+3,n]}_{[p+2,n-1]} + \det& U^{[p+2,n]}_{\{p\}\cup[p+2,n-1]} \det U^{\{p+1\}\cup[p+3,n]}_{[p+2,n]}=\\ = &\det U^{[p+2,n]}_{[p+2,n]} \det U^{\{p+1\}\cup[p+3,n]}_{\{p\}\cup[p+2,n-1]}.
\end{split}
\end{equation}
Combining the first and the third terms in Formula~\eqref{eq:complcso} via Formula~\eqref{eq:compldj} and dividing both sides by $(-1)^{n-p} \det U^{[q+1,n]}_{[q+1,n]}$, Formula~\eqref{eq:psisqm} follows.

\emph{Case $q-p = 1$, $q = n -1$.} In this case, the mutation at $\psi_{\square}$ reads
\begin{equation}\label{eq:complcss}
\psi_{\square}\psi_{\square}^{\prime} = h_{n-2,n}h_{n-1,n-1} + (h_{n-1,n}^{\prime})^{2}.
\end{equation}
Expanding the latter relation, we see that
\begin{equation}\begin{split}
\psi_{\square}(U) \psi_{\square}^{\prime}(U) = &u_{n-2,n} \left[\det U^{[n-1,n]}_{[n-1,n]} u_{nn} + \det U^{[n-1,n]}_{\{n-2\}\cup\{n\}}u_{n-1,n}\right] + \left[ \det U^{[n-1,n]}_{\{n-2\}\cup\{n\}}\right]^{2} = \\ = &u_{nn} \left[u_{n-2,n-1} \det U^{[n-1,n]}_{\{n-2\}\cup\{n\}} + u_{n-2,n} \det U^{[n-1,n]}_{[n-1,n]} \right].
\end{split}
\end{equation}
Dividing both sides by $\psi_{\square}(U) = u_{nn}$, we obtain Formula~\eqref{eq:psisqm}.

\emph{Case $q-p \neq 1$.} In this case, the mutation at $\psi_{\square}$ reads
\begin{equation}
\psi_{\square}\psi_{\square}^{\prime} = h_{p+1,p+2}^{\prime} h_{qq} h_{q+1,q+2} + h_{q,q+1} h_{p+1,p+1}.
\end{equation}
Expanding the right-hand side, we see that
\begin{equation}\label{eq:kakoet}
\begin{split}
(-1)^{n-q}\psi_{\square}(U)&\psi_{\square}^{\prime}(U) = \det U^{[p+1,n]}_{\{p\}\cup[p+2,n]} \det U^{[q,n]}_{[q,n]} \det U^{[q+2,n]}_{[q+1,n-1]} + \\ + & \det U^{[q+1,n]}_{[q,n-1]} \left[ \det U^{[p+1,n]}_{[p+1,n]} \det U^{[q+1,n]}_{[q+1,n]} + \det U^{[p+1,n]}_{\{p\}\cup[p+2,n]} \det U^{\{q\}\cup[q+2,n]}_{[q+1,n]}\right].
\end{split}
\end{equation}
Applying the Desnanot-Jacobi identity (see Proposition~\ref{p:dj22}) to the matrix $A:= U^{[q,n]}_{[q,n]}$, we see that
\begin{equation}\label{eq:kakoetj}
\det U^{[q,n]}_{[q,n]} \det U^{[q+2,n]}_{[q+1,n-1]} + \det U^{[q+1,n]}_{[q,n-1]} \det U^{\{q\}\cup [q+2,n]}_{[q+1,n]} = \det U^{[q+1,n]}_{[q+1,n]} \det U^{\{q\}\cup[q+2,n]}_{[q,n-1]}.
\end{equation}
Combining the first and the third terms in Formula~\eqref{eq:kakoet} with Formula~\eqref{eq:kakoetj} and dividing both sides by $(-1)^{n-q} \psi_{\square}$, one obtains Formula~\eqref{eq:psisqm}.
\end{proof}

\begin{lemma}\label{eq:basecoprim}
    The regular functions $\psi_{\square}$ and $\psi^\prime_{\square}$ are coprime.
\end{lemma}
\begin{proof}
    Evidently, $\psi_{\square}$ is irreducible, so it suffices to show that $\psi^{\prime}_{\square}(U)$ is not divisible by $\psi_{\square}(U)$. If $p+1 < q+1$, then $\psi_{\square}^{\prime}$ is generically nonzero on the variety given by $u_{n,q+1} = u_{n,q+2} = \cdots = u_{nn} = 0$, whereas $\psi_{\square}$ vanishes. If $p+1 > q+1$, then let $V$ be the variety given by the equations 
    \[
    u_{i,q+1} - u_{i,q+2} = 0, \ \ i \in [q+1,n].
    \]
    We see that $\psi_{\square}(U)|_{V} = 0$; on the other hand,
    \[
    \psi^{\prime}_{\square}(U)|_{V} = (-1)^{\varepsilon_{\square}} \det U^{[p+1,n]}_{\{p\}\cup[p+2,n]} \det U^{\{q\}\cup [q+2,n]}_{[q,n-1]}
    \]
    which is generically nonzero on $V$. Thus $\psi_{\square}$ and $\psi_{\square}^{\prime}$ are coprime.
\end{proof}

We shall use of the following lemma:
\begin{lemma}\label{l:transc}
Let $\mathcal{F}$ be a field of characteristic zero, and let $\alpha$ and $\beta$ be distinct transcendental elements over $\mathcal{F}$ such that $\mathcal{F}(\alpha) = \mathcal{F}(\beta)$. If there is a relation
\begin{equation}
    \sum_{k=1}^m (\alpha^k-\beta^k)p_k = 0
\end{equation}
for $p_k \in \mathcal{F}$, then all $p_k = 0$.
\end{lemma}
\begin{proof}
    See Lemma 5.15 in \cite{multdouble}.
\end{proof}

\begin{lemma}\label{l:fixptincl}
    For any $f \in \mathbb{C}[\GL_n]$, if $\mathcal{Q}^*(f) = f$, then $f \in \mathcal{L}_{\mathbb{C}}(\Psi^{\prime})$.
\end{lemma}
\begin{proof}
Since $\mathbb{C}[\GL_n] \subseteq \mathcal{L}_{\mathbb{C}}(\tilde{\Psi})$, one can find a sequence of elements $f_k \in \mathcal{L}_{\mathbb{C}}(\tilde{\Psi})$ that do not involve the variable $h_{p+1,p+1}$, such that
\begin{equation}\label{eq:ffkhp}
f(U) = \sum_{k \geq 0} f_{k}(U) [\tilde{h}_{p+1,p+1}(U)]^k.
\end{equation}
Note that $\tilde{h}_{p+1,p+1}$ is frozen in $\gc_h^{\dagger}(\bg_{\std})$, so the expression is polynomial in $\tilde{h}_{p+1,p+1}$. Applying $(\mathcal{F}^c)^*$ to~\eqref{eq:ffkhp} and using Lemma~\ref{l:relpsi} together with the assumption $(\mathcal{F}^c)^*(f) = f$ yields
\begin{equation}\label{eq:fffk}
f(U) = \sum_{k \geq 0} f_{k}(U) \left[\frac{h_{p+1,p+1}(U)}{\psi_{\square}(U)}\right]^k.
\end{equation}
Subtracting~\eqref{eq:ffkhp} from~\eqref{eq:fffk} and invoking Lemma~\ref{l:transc}, we conclude that $f(U) = f_0(U)$. Since $\tilde{\psi}_{\square}(U)$ is frozen in $\gc_h^{\dagger}(\bg_{\std})$, it enters $f_0(U)$ only with nonnegative exponents, so one can rewrite it in terms of a fraction with $\psi_{\square}^{\prime}$ in the denominator. Thus $f \in \mathcal{L}_{\mathbb{C}}(\Psi^{\prime})$.
\end{proof}

\begin{proposition}\label{p:baseshif}
Under the setup of the current subsection, the following statements hold:
\begin{enumerate}[1)]
    \item All the variables in $\Psi$ are regular and irreducible;
    \item For any cluster variable $\psi \in \Psi$, its mutation $\psi^\prime$ is regular and coprime with $\psi$;
    \item The generalized upper cluster structure $\bar{\mathcal{A}}_{\mathbb{C}}(\gc_h^{\dagger}(\bg))$ is naturally isomorphic to $\mathbb{C}[\GL_n]$.
\end{enumerate}
\end{proposition}
\begin{proof}
Clearly, $\psi_{\square}(U) = \det U^{[q+1,n]}_{[q+1,n]}$ is irreducible and coprime with $\psi_{\square}^{\prime}$ (it is possible to choose $U \in \GL_n$ such that $\psi_{\square}(U) = 0$ and such that each term in~\eqref{eq:psisqm} is positive). By Proposition~\ref{p:baseind}, it remains to show that $\mathbb{C}[\GL_n] \subseteq \mathcal{L}_{\mathbb{C}}(\Psi^{\prime})$. Since $\mathbb{C}[\GL_n] \subseteq \mathcal{L}_{\mathbb{C}}(\tilde{\Psi})$, it suffices to show that $\mathcal{L}_{\mathbb{C}}(\tilde{\Psi})\subseteq \mathcal{L}_{\mathbb{C}}(\Psi^{\prime})$; in turn, due to Lemma~\ref{l:relpsi}, proving the latter inclusion reduces to showing that $\det U^{[p+1,n]}_{[p+1,n]} \in \mathcal{L}_{\mathbb{C}}(\Psi^\prime)$. First, let us notice that
\begin{equation}\label{eq:fcqq}
(\mathcal{F}^c)^*\left( \det U^{\{q\}\cup [q+2,n]}_{I_{\square}}\right) = \det U^{\{q\}\cup [q+2,n]}_{I_{\square}},
\end{equation} 
where $I_{\square}$ is given by Formula~\eqref{eq:intsq}. This follows from the following observations: 
\begin{enumerate}[1)]
    \item The multiplication of $U$ by $\tilde{\gamma}^*(U_-)^{-1}$ on the right results in subtracting from the column $U^{\{p\}}$ the multiple $\alpha(U) \cdot U^{\{p+1\}}$. Since either $p+1\in \{q\}\cup [q+2,n]$ or $p \notin \{q\}\cup [q+2,n]$, we see that
    \[
    \det \left[U \tilde{\gamma}^*(U_-)^{-1}\right]^{\{q\}\cup[q+2,n]}_{I} = \det U^{\{q\}\cup[q+2,n]}_{I}
    \]
    for any $I \subseteq [1,n]$ of an appropriate size;
    \item Similarly, the multiplication of $U$ by $\tilde{\gamma}^*(U_-)$ on the left results in adding $\alpha(U)\cdot U_{\{p\}}$ to the row $U_{\{p+1\}}$. It is easy to see that if $q-p \neq 1$, then either $p+1 \notin I_{\square}$ or $p \in I_{\square}$; if $q-p = 1$, then always $p \in I_{\square}$; in both cases, 
    \[
    \det \left[\tilde{\gamma}^*(U_-)U\right]^J_{I_{\square}} = \det U^J_{I_{\square}}
    \]
    for any $J \subseteq [1,n]$ of an appropriate size.
\end{enumerate}
We conclude that Formula~\eqref{eq:fcqq} holds. By Lemma~\ref{l:fixptincl},  $\det U^{\{q\}\cup[q+2,n]}_{I_{\square}} \in \mathcal{L}_{\mathbb{C}}(\Psi^{\prime})$. Now, notice that $\det U^{[q+1,n]}_{I_{\square}}$ is a cluster variable in $\Psi^{\prime}$ (hence an invertible element of $\mathcal{L}_{\mathbb{C}}(\Psi^{\prime})$), for
\[
\det U^{[q+1,n]}_{I_{\square}} = \begin{cases}
    (-1)^{n-q} h_{q,q+1}(U) \ &\text{if} \ q-p \neq 1;\\
    (-1)^{n-p} h^{\prime}_{p+1,p+3}(U) \ &\text{if}\ q-p = 1, \ p \leq n-3;\\
    (-1)^{n-p} h_{pn}(U) \ &\text{if} \ q-p = 1, \ p = n-2.
\end{cases}
\]
It follows that one can solve for $\det U^{[p+1,n]}_{[p+1,n]}$ in the ring $\mathcal{L}_{\mathbb{C}}(\Psi^{\prime})$ from Formula~\eqref{eq:psisqm}. Due to the discussion in the beginning of the proof, we finally conclude that the statement holds.
\end{proof}

\subsection{The case of $|\Gamma_1|=|\Gamma_2| = 1$ (initial cluster).}
Although in the previous subsection we proved  $\bar{\mathcal{A}}(\gc_h^{\dagger}(\bg)) = \mathbb{C}[\GL_n]$ for $\bg = (\Gamma_1,\Gamma_2,\gamma)$ with $|\Gamma_1| = 1$, we proved regularity, irreducibility and coprimality with mutations not in the initial extended cluster $\Psi_0$, but in a certain shifted extended cluster $\Psi$. According to Proposition~\ref{p:baseind}, in order to claim the same properties for $\Psi_0$, we need to verify them for the marked variable. As in the previous section, let us assume that $\Gamma_1 = \{p\}$ and $\Gamma_2 = \{q\}$. Then there is only one marked variable given by $\psi_{\square} = h_{q+1,q+1}$.

\begin{lemma}\label{l:inimarked}
The mutation of $\Psi_0$ at the marked variable $\psi_{\square}$ produces the variable
%\begin{equation}
\[
\psi_{\square}^\prime(U) = \begin{cases} 
(-1)^{p+q+1} \left[ u_{p+1,n}\det U^{[q+1,n]}_{[q,n-1]}  + u_{pn}\det U^{\{q\}\cup[q+2,n]}_{[q,n-1]}  \right] \  &q\neq p+1;\\[10pt]
\det U^{[q+1,n]}_{[q+1,n]}\left[ u_{p+1,n}\det U^{[q+1,n]}_{[q,n-1]}  + u_{pn}\det U^{\{q\}\cup[q+2,n]}_{[q,n-1]}  \right] + \\[7pt] + \det U^{\{q\}\cup[q+2,n]}_{[q+1,n]}\left[u_{p+1,n}\det U^{[q+1,n]}_{\{q-1\}\cup[q+1,n-1]} + u_{pn} \det U^{\{q\}\cup[q+2,n]}_{\{q-1\}\cup[q+1,n-1]}  \right] \ &q = p+1.
\end{cases}
\]
%\end{equation}
\end{lemma}
\begin{proof}
The exchange relation is
\[
\psi_{\square}\psi_{\square}^\prime = h_{q,q+1} h_{p+1,n} + h_{qq} h_{pn} h_{q+1,q+2}.
\]
Let us study two cases:

\emph{Case $q \neq p+1$.} Writing out all the functions, the relation becomes
\begin{equation}\label{eq:abca}
\begin{split}
(-1)^{p+q+1}\psi_{\square}(U) \psi_{\square}^\prime(U) = \det & U^{[q+1,n]}_{[q,n-1]} u_{p+1,n} \det U^{[q+1,n]}_{[q+1,n]} + \\ + &u_{pn} \left(\det U^{[q+1,n]}_{[q,n-1]} \det U^{\{q\}\cup [q+2,n]}_{[q+1,n]} + \det U^{[q,n]}_{[q,n]} \det U^{[q+2,n]}_{[q+1,n-1]} \right).
\end{split}
\end{equation}
Applying the Desnanot-Jacobi relation (see Proposition~\ref{p:dj22}) to the last term, we see that 
\[
\det U^{[q+1,n]}_{[q,n-1]} \det U^{\{q\}\cup [q+2,n]}_{[q+1,n]} + \det U^{[q,n]}_{[q,n]} \det U^{[q+2,n]}_{[q+1,n-1]} = \det U^{[q+1,n]}_{[q+1,n]} \det U^{\{q\}\cup [q+2,n]}_{[q,n-1]};
\]
hence, after dividing both sides by $\det U^{[q+1,n]}_{[q+1,n]}$ in~\eqref{eq:abca}, the result follows.

\emph{Case $q = p+1$.} Writing out all functions and rearranging the terms, the relation becomes
\begin{equation}\label{eq:mutq1e}
\begin{split}
\psi_{\square}^\prime(U) = u_{p+1,n}&\left[ \det U^{[q+1,n]}_{[q+1,n]} \det U^{[q+1,n]}_{[q,n-1]} + \det U^{[q+1,n]}_{\{q-1\}\cup[q+1,n-1]} \det U^{\{q\}\cup[q+2,n]}_{[q+1,n]} \right] + \\ + u_{pn} &\left[\det U^{[q+1,n]}_{[q,n-1]} \det U^{\{q\}\cup[q+2,n]}_{[q+1,n]} + \det U^{[q,n]}_{[q,n]} \det U^{[q+2,n]}_{[q+1,n-1]} \right] +\\+&  \frac{u_{pn} \det U^{\{q\}\cup[q+2,n]}_{[q+1,n]}}{\det U^{[q+1,n]}_{[q+1,n]}} \cdot A
\end{split}
\end{equation}
where $A$ is given by
\begin{equation}\label{eq:mutae}
A =  \det U^{[q+1,n]}_{\{q-1\}\cup[q+1,n-1]} \det U^{\{q\}\cup[q+2,n]}_{[q+1,n]} + \det U^{[q,n]}_{\{q-1\}\cup [q+1,n]} \det U^{[q+2,n]}_{[q+1,n-1]}.
\end{equation}
The second term in~\eqref{eq:mutq1e} can be simplified via the Desnanot-Jacobi identity as %(see Proposition~\ref{p:dj22}):
\[
\det U^{[q+1,n]}_{[q,n-1]} \det U^{\{q\}\cup[q+2,n]}_{[q+1,n]} + \det U^{[q,n]}_{[q,n]} \det U^{[q+2,n]}_{[q+1,n-1]} = \det U^{[q+1,n]}_{[q+1,n]} \det U^{\{q\}\cup[q+2,n]}_{[q,n-1]};
\]
likewise, Formula~\eqref{eq:mutae} can be simplified as
\[\begin{split}\det U^{[q+1,n]}_{\{q-1\}\cup[q+1,n-1]}\det U^{\{q\}\cup[q+2,n]}_{[q+1,n]} +  \det& U^{[q,n]}_{\{q-1\}\cup [q+1,n]} \det U^{[q+2,n]}_{[q+1,n-1]} =\\= &\det U^{[q+1,n]}_{[q+1,n]} \det U^{\{q\}\cup[q+2,n]}_{\{q-1\}\cup[q+1,n-1]}.
\end{split}
\]
Combining the above terms, the formula for $\psi_{\square}^\prime$ follows.
\end{proof}

\begin{proposition}\label{p:baseini}
Under the setup of the current subsection, the following statements hold:
    \begin{enumerate}[1)]
    \item All the variables in $\Psi_0$ are regular and irreducible;
    \item For any cluster variable $\psi \in \Psi_0$, its mutation $\psi^\prime$ is regular and coprime with $\psi$.
    \end{enumerate}
\end{proposition}
\begin{proof}
    According to Proposition~\ref{p:baseind}, it is enough to verify the above statements only for $\psi_{\square}$. Evidently, $\psi_{\square}$ is irreducible and $\psi_{\square}^{\prime}$ is regular (see Lemma~\ref{l:inimarked}). If $q \neq p+1$, we see that $\psi_{\square}$ vanishes on the variety given by $u_{n,q+1} = u_{n,q+2} = \cdots = u_{nn} = 0$, whereas $\psi_{\square}^\prime(U)$ is generically nonzero. If $q = p+1$, then it suffices only to check that
    \begin{equation}\label{eq:irrpiecec}
        u_{p+1,n}\det U^{[q+1,n]}_{\{q-1\}\cup[q+1,n-1]} + u_{pn} \det U^{\{q\}\cup[q+2,n]}_{\{q-1\}\cup[q+1,n-1]}  
    \end{equation}
    is not divisible by $\psi_{\square}(U)$, which immediately follows from the same argument.
\end{proof}


\subsection{The general case}
In this subsection, we finalize the proofs of Part~\ref{i:gln_ni} of Theorem~\ref{thm:maingln} and Part~\ref{i:sln_ni} of Theorem~\ref{thm:mainsln}.

\begin{proposition}\label{p:compl}
    Let $\bg = (\Gamma_1,\Gamma_2,\gamma)$ be any BD triple of type $A_{n-1}$, and let $G \in \{\GL_n(\mathbb{C}),\SL_n(\mathbb{C})\}$. Then the following statements hold:
    \begin{enumerate}[1)]
    \item The generalized cluster structure $\gc_h^{\dagger}(\bg)$ is regular;
    \item All the variables in the initial extended cluster of $\gc_h^{\dagger}(\bg,G)$ are irreducible (as elements of $\mathcal{O}(G)$) and (for cluster variables) coprime with their mutations;
    \item The generalized upper cluster algebra of $\gc_h^{\dagger}(\bg,G)$ is naturally isomorphic to $\mathcal{O}(G)$.
    \end{enumerate}
\end{proposition}
\begin{proof}
As in the previous papers~\cite{plethora,multdouble}, we run an induction on the size $|\Gamma_1|$ for a fixed $n$. For $|\Gamma_1| = 0$, the statement was proved in~\cite{double}; for $|\Gamma_1| = 1$, the statement is contained in Proposition~\ref{p:baseshif} and Proposition~\ref{p:baseini}. For $|\Gamma_1| > 1$, the statement follows from the existence of birational quasi-isomorphisms with disjoint sets of marked variables and Proposition~\ref{p:stepind}.
\end{proof}

==> p_toric.tex <==
In this subsection, for any BD triple $\bg = (\Gamma_1,\Gamma_2,\gamma)$ of type $A_{n-1}$, we show that the action (...) defines a global toric action on $\gc_h^{\dagger}(\bg)$.
